Human Choice Prediction in Language-based Persuasion Games: Simulation-based Off-Policy Evaluation

Recent advances in Large Language Models (LLMs) have spurred interest in designing LLM-based agents for tasks that involve interaction with human and artificial agents. This paper addresses a key aspect in the design of such agents: predicting human decisions in off-policy evaluation (OPE). We focus on language-based persuasion games, where an expert aims to influence the decision-maker through verbal messages. In our OPE framework, the prediction model is trained on human interaction data collected from encounters with one set of expert agents, and its performance is evaluated on interactions with a different set of experts. Using a dedicated application, we collected a dataset of 87K decisions from humans playing a repeated decision-making game with artificial agents. To enhance off-policy performance, we propose a simulation technique involving interactions across the entire agent space and simulated decision-makers. Our learning strategy yields significant OPE gains, e.g., improving prediction accuracy in the top 15% challenging cases by 7.1%. Our code and the large dataset we collected and generated are submitted as supplementary material and publicly available in our GitHub repository: https://github.com/eilamshapira/HumanChoicePrediction

==> 91.Algorithem_Apendex.tex <==

\section{Simulation Pseudo Code}
\label{appendix:pseudocode}

\input{pseudocode/simulation}


==> 99.refrences.tex <==
% \section*{References}

% \medskip

% {
% \small

% [1] Bousmalis, Konstantinos, Alex Irpan, Paul Wohlhart, Yunfei Bai, Matthew Kelcey, Mrinal Kalakrishnan, Laura Downs et al. "Using simulation and domain adaptation to improve efficiency of deep robotic grasping." In 2018 IEEE international conference on robotics and automation (ICRA), pp. 4243-4250. IEEE, 2018.

% [2] Vacaro, Juliano, Guilherme Marques, Bruna Oliveira, Gabriel Paz, Thomas Paula, Wagston Staehler, and David Murphy. "Sim-to-real in reinforcement learning for everyone." In 2019 Latin American Robotics Symposium (LARS), 2019 Brazilian Symposium on Robotics (SBR) and 2019 Workshop on Robotics in Education (WRE), pp. 305-310. IEEE, 2019.

% [3] Tesauro, Gerald. "Practical issues in temporal difference learning." Advances in neural information processing systems 4 (1991).

% [4] Yue, Xiangyu, Bichen Wu, Sanjit A. Seshia, Kurt Keutzer, and Alberto L. Sangiovanni-Vincentelli. "A lidar point cloud generator: from a virtual world to autonomous driving." In Proceedings of the 2018 ACM on International Conference on Multimedia Retrieval, pp. 458-464. 2018.

% [5] Gao, Ge, Song Ju, Markel Sanz Ausin, and Min Chi. "Hope: Human-centric off-policy evaluation for e-learning and healthcare." arXiv preprint arXiv:2302.09212 (2023).

% [6] Sharma, Archit, Michael Ahn, Sergey Levine, Vikash Kumar, Karol Hausman, and Shixiang Gu. "Emergent real-world robotic skills via unsupervised off-policy reinforcement learning." arXiv preprint arXiv:2004.12974 (2020).

% [7] Kahn, H., Marshall, A. W. (1953). Methods of reducing sample size in Monte Carlo computations. In Journal of the Operations Research Society of America, 1(5):263–278.

% [8] Dudík, Miroslav, John Langford, and Lihong Li. "Doubly robust policy evaluation and learning." arXiv preprint arXiv:1103.4601 (2011).

% [9] Uehara, Masatoshi, Chengchun Shi, and Nathan Kallus. "A Review of Off-Policy Evaluation in Reinforcement Learning." arXiv preprint arXiv:2212.06355 (2022).

% [10] Rubinstein, R. Y. (1981). Simulation and the Monte Carlo Method, New York, Wiley.

% [11] Koller, D., Friedman, N. (2009). Probabilistic Graphical Models: Principles and Techniques. MIT Press, 2009.

% [12] Raifer, Maya, Guy Rotman, Reut Apel, Moshe Tennenholtz, and Roi Reichart. "Designing an automatic agent for repeated language–based persuasion games." Transactions of the Association for Computational Linguistics 10 (2022): 307-324.

% [13] Apel, Reut, Ido Erev, Roi Reichart, and Moshe Tennenholtz. "Predicting decisions in language based persuasion games." Journal of Artificial Intelligence Research 73 (2022): 1025-1091.

% [14] Bewley, Alex, Jessica Rigley, Yuxuan Liu, Jeffrey Hawke, Richard Shen, Vinh-Dieu Lam, and Alex Kendall. "Learning to drive from simulation without real world labels." In 2019 International conference on robotics and automation (ICRA), pp. 4818-4824. IEEE, 2019.

% [15] Calderon, Nitay, Eyal Ben-David, Amir Feder, and Roi Reichart. "Docogen: Domain counterfactual generation for low resource domain adaptation." arXiv preprint arXiv:2202.12350 (2022).

% [16] Cao, Minh, and Ramin Ramezani. "Data generation using simulation technology to improve perception mechanism of autonomous vehicles." arXiv preprint arXiv:2207.00191 (2022).

% [17] Graves, Alex, and Alex Graves. "Long short-term memory." Supervised sequence labelling with recurrent neural networks (2012): 37-45.

% [18] Yue, Xiangyu, Bichen Wu, Sanjit A. Seshia, Kurt Keutzer, and Alberto L. Sangiovanni-Vincentelli. "A lidar point cloud generator: from a virtual world to autonomous driving." In Proceedings of the 2018 ACM on International Conference on Multimedia Retrieval, pp. 458-464. 2018.

% [19] Saadallah, Amal, Felix Finkeldey, Jens Buß, Katharina Morik, Petra Wiederkehr, and Wolfgang Rhode. "Simulation and sensor data fusion for machine learning application." Advanced Engineering Informatics 52 (2022): 101600.

% [20] Kamenica, Emir, and Matthew Gentzkow. "Bayesian persuasion." American Economic Review 101, no. 6 (2011): 2590-2615.

% [21] Aumann, Robert J., Michael Maschler, and Richard E. Stearns. Repeated games with incomplete information. MIT press, 1995.

% [22] Kahneman, Daniel, and Amos Tversky. "Prospect theory: An analysis of decision under risk." In Handbook of the fundamentals of financial decision making: Part I, pp. 99-127. 2013.
% % [1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms for
% % connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and T.K.\ Leen
% % (eds.), {\it Advances in Neural Information Processing Systems 7},
% % pp.\ 609--616. Cambridge, MA: MIT Press.


% % [2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS: Exploring
% %   Realistic Neural Models with the GEneral NEural SImulation System.}  New York:
% % TELOS/Springer--Verlag.


% % [3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of learning and
% % recall at excitatory recurrent synapses and cholinergic modulation in rat
% % hippocampal region CA3. {\it Journal of Neuroscience} {\bf 15}(7):5249-5262.

% }

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> ICLR-WS/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> figures/a-game.tex <==
\begin{figure}
  \centering
  \fbox{ % \rule[-.5cm]{0cm}{4cm} 
  \includegraphics[width=12cm]{figures/a-game.png}
  %\rule[-.5cm]{4cm}{0cm}
  }
  % \caption{Data of a game. For each round, we use features of the verbal signal sent by the expert and features about the last action taken by the DM in the previous round and its results to predict if the player will choose to go to this hotel or stay at home.}
  \caption{The game data. We use features of the verbal signal sent by the expert and features about the previous round's action, result, and reaction time to predict whether the player will choose to go to the hotel or stay at home.}
\label{fig:a-game}
\end{figure}


==> figures/review.tex <==
\begin{figure}[htp]
  \centering
  \fbox{ % \rule[-.5cm]{0cm}{4cm} 
  \includegraphics[width=13cm]{figures/a-review-2.png}
  %\rule[-.5cm]{4cm}{0cm}
  }
  \caption{A sample review from our hotel review dataset.}
    \label{fig:review}

\end{figure}


==> figures/what_improves.tex <==
\begin{figure*}[htp]
 
  \centering
  \fbox{
  \includegraphics[width=13.4cm]{figures/fig4_final.png}
}

  \caption{Ablation analysis of the impact of the different components of the simulation. We consider the simulation without the behavioral and textual components ($p_1 = p_2 = 0$, V2), or when the simulated DM does not improve over time ($\eta = 0$, V3), or when the experts in the simulation are the  $E_\mathcal{B}$ strategies (V4).
  Top: All examples. Bottom: challenging examples for Majority.}
\label{what-improves}
\end{figure*}


==> pseudocode/simulation.tex <==
\begin{algorithm}
\caption{Simulate DM data}\label{alg:simulation}
\begin{algorithmic}
    
    \Require the functions $generate\_nature\_vector()$, $play\_round(user, bot)$, $get\_random\_bots()$
    \Procedure {$update\_temperament$}{$user$}
    \For{$i$ in \{1..3\}}

    \State \texttt{$\gamma_i \gets Uni(-\frac{\eta}{10}, \frac{9 \eta}{10})$}
    \State \texttt{$user.temperament\_vector[i] \gets (1 - \gamma_i) \cdot user.temperament\_vector[i]  $}
    \EndFor
    \If {$\sum_{1 \le i \le 3} user.temperament\_vector[i] > 1$}
        \State \texttt{$normalization\_factor \gets \sum_{1 \le i \le 3} user.temperament\_vector[i] $}
        \For{$i$ in \{1..3\}}
        \State \texttt{$user.temperament\_vector[i] \gets  \frac{user.temperament\_vector[i]}{normalization\_factor}$}
        \EndFor
    \EndIf
    \State \texttt{$user.temperament\_vector[0] \gets 1 - \sum_{1 \le i \le 3} user.temperament\_vector[i]$}
    \
    \EndProcedure

    \Procedure {$generate\_DM\_data(user)$}{}
    \State \texttt{$user.nature\_vector \gets generate\_nature\_vector()$}
    \State \texttt{$user.rivals \gets get\_random\_bots() $}

    \For{$bot$ in $user.rivals$}
        \State \texttt{$user.temperament\_vector \gets (0, user.nature\_vector)$}
        \State \texttt{$user.game\_points = 0$}
         \While{$user.game\_points < 9$}
         \State \texttt{$user.temperament\_vector \gets (0, user.nature\_vector)$}
         \For{round in \{1..10\}}
            \State \texttt{$play\_round(user, bot)$}
            \State \texttt{$update\_temperament(user)$}
         \EndFor
        \EndWhile
    \EndFor
    \EndProcedure

\end{algorithmic}
\end{algorithm}

==> pseudocode/training_process.tex <==
\begin{algorithm}
\caption{Training Loop}\label{alg:deep_training}
\begin{algorithmic}
\Require interaction\_train\_dataset
% \If {do\_initialisation\_simulation}
\State \texttt{ pre\_training\_DS = Create\_Simulation\_Dataset(n\_players = $S_{pt}$)} 
\State \texttt{ model.train(dataset = initialization\_DS) } \Comment{ Training with pre-training simulation} 
% \EndIf
\For{\texttt{$epoch \gets 1$ to $N_{epochs}$}}
%\If {do\_online\_simulation}
    \State \texttt{ epoc\_DS = Create\_Simulation\_Dataset(n\_players = $S_{e}$)}
    \State \texttt{ model.train(dataset = online\_DS) } \Comment{Training with epoch simulation}
%    \EndIf
    \State \texttt{ model.train(dataset = interaction\_train\_dataset) }  
\EndFor
\end{algorithmic}
\end{algorithm}

==> tables/accuracy-by-strategy.tex <==
\begin{table*}[t]
  \label{accuracy-by-strategy}
  \centering
  \begin{tabular}{llllllll} 
    \hline
    % strategy        & \#132             & \#23               & \#107              & \#43               & \#17               & \#93               & Mean              \\
    Model \symbol{92} Expert       & \#1             & \#2               & \#3              & \#4               & \#5               & \#6               & Average              \\
    \hline
LSTM+S & 85.47\% & \textbf{80.93\%} & \textbf{90.27\%} & \textbf{82.51\%} & \textbf{79.66\%} & \textbf{86.71\%} & \textbf{84.26\%} \\
LSTM & 84.59\% & 80.12\% & 88.88\% & 82.12\% & 78.59\% & 85.17\% & 83.24\% \\
LSTM OS & 84.85\% & 71.63\% & 87.22\% & 76.38\% & 71.15\% & 81.38\% & 78.77\% \\
XGBoost+S & \textbf{86.13\%} & 78.82\% & 88.68\% & 82.3\% & 77.92\% & 86.46\% & 83.38\% \\
XGBoost & 85.43\% & 78.72\% & 87.82\% & 82.32\% & 76.23\% & 86.1\% & 82.77\% \\
TF+S & 84.38\% & 78.3\% & 88.57\% & 81.71\% & 77.07\% & 84.54\% & 82.43\% \\
TF & 84.26\% & 78.83\% & 87.67\% & 81.35\% & 76.61\% & 84.88\% & 82.27\% \\
Majority & 85.13\% & 72.2\% & 85.89\% & 79.06\% & 70.72\% & 80.46\% & 78.91\% \\
% \bottomrule
  \end{tabular}

  \begin{tabular}{llllllll}
\hline
\hfill \symbol{92} Hard to & Maj. & XGBoost & LSTM+S & LSTM & TF & All  & One  \\
Accuracy of \symbol{92} &  &  & && & Baselines  & Baseline \\
\hline
LSTM+S & \textbf{70.55\%} & \textbf{72.15\%} & \textbf{61.68\%} & \textbf{64.56\%} & \textbf{66.45\%} & \textbf{59.68\%} & \textbf{72.74\%} \\
LSTM & 67.76\% & 67.44\% & 57.16\% & 58.69\% & 62.01\% & 56.17\% & 70.11\% \\
XGBoost+S & 68.66\% & 68.26\% & 60.72\% & 62.9\% & 62.56\% & 57.64\% & 71.09\% \\
XGBoost & 66.82\% & 65.6\% & 60.22\% & 62.26\% & 62.53\% & 54.43\% & 69.9\% \\
TF+S & 66.45\% & 66.18\% & 57.4\% & 59.11\% & 59.87\% & 56.77\% & 68.97\% \\
TF & 66.1\% & 66.3\% & 55.86\% & 58.4\% & 59.39\% & 56.86\% & 68.44\% \\
Majority & 62.43\% & 63.37\% & 58.08\% & 59.67\% & 58.57\% & 55.17\% & 64.67\% \\
\hline
\# Decisions & 3568 & 4490 & 3898 & 4085 & 4502 & 957 & 7694 \\
\% tot. Dec. & 24.99\% & 31.44\% & 27.3\% & 28.61\% & 31.53\% & 6.7\% & 53.88\% \\
%\% Decisions &  &  &  &  &  &  &  \\
\hline
\end{tabular}
\caption{Top: Average accuracy of each model by expert strategy (Q1 and Q2), with "+S" indicating models trained using both simulation and interaction data. TF = Transformer. Maj = Majority. LSTM OS = LSTM trained with simulation data only. The best-performing model is highlighted in bold. Expert strategies are listed in the order of their appearance during the game. Bottom: Performance of the various models when predicting decisions where the confidence level of the column model is at least 20\% for both classes. The results demonstrate that incorporating simulated interactions in the training process improves the accuracy of the models for each subset of challenging decisions, as compared to model variants that are trained with human-bot interactions only. }
\end{table*}


==> tables/feature_types.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Simulation Factor & BERT & GPT4 & EF \\ \hline
0.0               & -67.9\%  & 32.6\% & 0.0\%  \\ \hline
0.5               & -7.2\%  & 40.6\% & 6.8\%  \\ \hline
1.0               & 22.7\%  & 69.0\% & 33.7\%  \\ \hline
1.5               & 33.4\%  & \bestResult{69.8\%} & 65.6\%  \\ \hline
2.0               & \bestResult{33.7\%}  & 59.7\% & 83.2\%  \\ \hline
3.0               & 27.3\%  & 41.2\% & 92.6\%  \\ \hline
4.0               & 6.0\%  & 19.1\% & \bestResult{100.0\%}  \\ \hline
\end{tabular}

==> tables/hard-decisions-0.25.tex <==
\begin{table}
  \caption{Performance of the various models when predicting decisions where the confidence level of the model at the top of the column is less than 20\%. The results demonstrate that incorporating simulation techniques in the prediction process improved the accuracy of the models for each subset of challenging decisions, as compared to the other models.}
  \label{hard-decisions-0.25}
  \centering

\begin{tabular}{llllllll}
\toprule
\hfill \symbol{92} Hard to & Majorirty & XGBoost & LSTM+S & LSTM & Trans. & all  & one  \\
Accuracy of \symbol{92} &  &  & && & baselines  & baseline \\
\midrule
LSTM+S & \textbf{70.55\%} & \textbf{72.15\%} & \textbf{61.68\%} & \textbf{64.56\%} & \textbf{66.69\%} & \textbf{60.34\%} & \textbf{72.78\%} \\
XGBoost+S & 68.66\% & 68.26\% & 60.72\% & 62.9\% & 64.11\% & 57.72\% & 71.17\% \\
LSTM & 67.76\% & 67.44\% & 57.16\% & 58.69\% & 61.68\% & 54.95\% & 70.23\% \\
XGBoost & 66.82\% & 65.6\% & 60.22\% & 62.26\% & 64.19\% & 55.63\% & 70.03\% \\
Transformer+S & 66.72\% & 67.4\% & 56.69\% & 60.55\% & 60.72\% & 53.65\% & 69.36\% \\
Transformer & 66.35\% & 67.1\% & 55.8\% & 58.54\% & 59.97\% & 55.28\% & 68.93\% \\
majority & 62.43\% & 63.37\% & 58.08\% & 59.67\% & 60.03\% & 56.94\% & 64.8\% \\
\midrule
\# of Decisions  & 3568 & 4490 & 3898 & 4085 & 4876 & 964 & 7834 \\
\% tot. Decisions & 24.99\%&	31.44\%&	27.30\%&	28.61\%&	34.15\%&	6.75\%&	54.86\% \\

\bottomrule

  \end{tabular}
\end{table}

